Salient Store: Enabling Smart Storage for Continuous Learning Edge Servers

As continuous learning based video analytics continue to evolve, the role of efficient edge servers in efficiently managing vast and dynamic datasets is becoming increasingly crucial. Unlike their compute architecture, storage and archival system for these edge servers has often been under-emphasized. This is unfortunate as they contribute significantly to the data management and data movement, especially in a emerging complute landscape where date storage and data protection has become one of the key concerns. To mitigate this, we propose Salient Store that specifically focuses on the integration of Computational Storage Devices (CSDs) into edge servers to enhance data processing and management, particularly in continuous learning scenarios, prevalent in fields such as autonomous driving and urban mobility. Our research, gos beyond the compute domain, and identifies the gaps in current storage system designs. We proposes a framework that aligns more closely with the growing data demands. We present a detailed analysis of data movement challenges within the archival workflows and demonstrate how the strategic integration of CSDs can significantly optimize data compression, encryption, as well as other data management tasks, to improve overall system performance. By leveraging the parallel processing capabilities of FPGAs and the high internal bandwidth of SSDs, Salient Store reduces the communication latency and data volume by ~6.2x and ~6.1x, respectively. This paper provides a comprehensive overview of the potential of CSDs to revolutionize storage, making them not just data repositories but active participants in the computational process.

==> src/04ExemplarSelction.tex <==
%%%%%%

The challenge of data drift in ML, where live data diverges from original training data, necessitates a robust exemplar selection mechanism in storage servers~\cite{ekya, UrbanTraffic, kitti, nuscenes, UrbanSound}. Our experimental investigations reveal that data drift can lead to significant degradation in network accuracy. A critical concern in this regard is the sampling bias~\cite{samplingbias} inherent in conventional exemplar selection methods. Such bias can result in model over-fitting for frequently-occurring classes while forgetting rare but crucial ones. 

To address these issues, we employ a representation learning framework~\cite{icarl} for effective exemplar selection. This approach involves using large DNN models as feature extractors to transform data into feature vectors, which are then clustered (e.g., using K-means~\cite{icarl}). The clustering process involves calculating the distance of new data from existing cluster centers, categorizing the data into one of three cases: i) known classes (similar to training samples), ii) known classes with significant differences (distillation loss~\cite{icarl}), or iii) entirely new classes (classification loss~\cite{icarl}). This methodology enables the identification of truly representative exemplars, minimizing data drift by ensuring the training data encompasses {\em both} existing and novel scenarios.

In our system, exemplar selection is further enhanced by employing custom hardware in the CSDs. Multiple ``teacher models'' contribute to creating a diverse and unbiased exemplar set. This set becomes the basis for continuous learning, effectively minimizing data drift. Once the newer model is trained with these exemplars, the data is discarded, and the teacher models' feature space is updated, ensuring both models remain current. The utilization of efficient hardware accelerators designed for intermittent power sources is crucial in this process, allowing for sustainable and efficient operations in storage servers.


\subsection{Design and Architecture of Exemplar Selection Hardware}
The SALT storage system's hardware design incorporates a sophisticated exemplar selection mechanism, crucial for addressing data drift in machine learning applications. This design aims to optimize data movement and power consumption without compromising throughput. To perform feature extraction using a CNN, our design implements a systolic array structure, which comprises 64 tiles arranged in an \(8\times8\) configuration. Each tile has 32-bit floating-point MAC units, which are ideal for convolution operations. This modular architecture allows for scalable compute in response to resource availability and compute demand. The system also includes a 1kB state buffer for state saving and data backup in case of servicing external interrupts or disk failure.

In our hardware design, a modular computational approach is central to the architecture. Each tile within the system is designated to process one kernel. This necessitates \(\lceil[C \times H \times W]/64\rceil\) iterations for handling a kernel of size \([C \times H \times W]\). To support data streaming and partial compute storage, the system incorporates four double-buffered Static Random-Access Memory (SRAM) structures. The weights in the network are stored in a double-buffered, multi-banked SRAM. This filter SRAM is divided into 64 banks, correlating with the number of tiles, with each bank having a capacity of 1kB. The management of input data broadcast across all tiles is executed via a 64kB double-buffered input feature map SRAM, with each half being 16kB. The full input loading requires \(\lceil [X \times Y \times Z]/1024 \rceil\) iterations, with each buffer undergoing \( [X \times Y \times Z]/2048 \) loading cycles. The convolution operation, transforming the input tensor \([X \times Y \times Z]\) to an output tensor \([M \times U \times V]\) using a kernel of size \([M \times C \times W \times H]\), is facilitated by this architecture. This transformation is expressed as \( [X \times Y \times Z] \xrightarrow{M \times C \times W \times H} [M \times U \times V] \). The output tensor dimensions \([M \times U \times V]\) are supported by a double-buffered output feature map SRAM, each bank being 1kB in size. Additionally, a 64kB SRAM is utilized as a scratchpad memory, which is essential for storing activations, transposes, and intermediate differentials during the backward pass of DNN training. The accelerator is also equipped with \(8 \times 8\) compactor-mux combinational logic units, each tile containing 64 units. These units are employed for ReLU activation in the forward pass and inverse activation in the backward pass. For scenarios involving smaller DNNs, where not all layers comprise 64 kernels, the system operates in a batching mode. The batch size, denoted as \( B \), is determined by \( B = \lfloor A/L \rfloor \), where \( L \) represents the layer with the fewest channels, and \( A \) is the total number of active tiles. This flexible design allows for adaptation to various workload requirements\footnote{Considering CNN acceleration on FPGAs with the help of systolic arrays is a well studied topic, we do not delve into much details of how the data flow is orchestrated, but we only limit our discussion to the hardware specification.}.

The software design ensures the data flow from the disks to the storage controller where the stripped data is stitched together (this can easily be done on CSDs as well, but considering the smaller footprint, and capabilities along with the efficiency of the commercial software for this we chose to use the software based solution for stitching the data) and then sent to the CSDs for feature extraction. Depending upon the data type, different models are invoked to perform convolution operations to provide with a feature vector. The resultant feature vectors are stored in the CSD and finally are clustered using k-means++~\cite{kmeanspp, kmeansppS} for finding the exemplar. The k-means algorithm, thanks to it's recursive nature, is hard to accelerate using FPGAs and hence is implemented using the software stack on the storage controller. Finally, each of these feature vector is tagged as true exemplar or false exemplar and the data read request from the compute servers is only handed over the data which are considered to be true exemplars. 

However, we are still left with one challenge. After the data are stitched, they still need to be decrypted before they could be used for exemplar selection. Moreover, as we are designing ML storage servers which are used for long-term storage, it is important to keep the data secure. However, the current state-of-the-art algorithms like RSA~\cite{rsa} have been proven not to be safe, especially with the advent of quantum computation~\cite{lattice02}. Towards this, we focus on the modern, post quantum, lattice based encryption~\cite{lattice02} and implementing them on the CSDs to make SALT future safe.

==> src/05DesignImplementation.tex <==
\subsection{Component Integration in SALT}
This section delves into the intricacies of how various components of the SALT storage system are cohesively integrated, detailing the implementation strategies and the orchestration of compute tasks. As illustrated in Fig.~\ref{fig:CompleteFlow}, SALT distinguishes between the write and read paths in the storage server. Classical optimizations for compression and RAID operations~\cite{h264, octtree, raid, unraid, zstd, minitool}, traditionally executed on CPUs, are incorporated within the storage controller. For encryption, we deviate from conventional RSA methods, opting instead for lattice-based encryption as outlined in Section~\ref{sec:SE}. The encryption process leverages the Vitis library~\cite{vitis}, employing High-Speed Schoolbook Polynomial Multiplication (HSPM) and Systolic Dimension Modular Multiplier (SDMM), both implemented in OpenCL and structured as systolic arrays, akin to CNNs. These components are synthesized for FPGA implementation using Vitis High-Level Synthesis (HLS). Additionally, Vitis Level-1 and Level-2 primitives~\cite{l1vitis} are utilized to enhance the efficiency of HSPM and SDMM implementations.

\begin{figure}[!htbp]
\centering 
\includegraphics[width=\linewidth]{figs/CompleteFlow.pdf}
\caption{Overall data-flow and compute mapping in the SALT storage system.}
\label{fig:CompleteFlow}
\end{figure}

\subsection{Read and Write Pathways}
Upon a read request for training, the data aggregation is managed using Minitool~\cite{minitool}. The decryption hardware, similar in design to the encryption hardware, is built with the Vitis HLS tool. Post decryption, data inflation is executed using standard industry tools~\cite{h264, octtree}. For exemplar selection on the storage servers, we have integrated a systolic array-based CNN accelerator into the CSD FPGA. This accelerator, as discussed in Section~\ref{sec:Exm}, is built using Vitis HLS, optimized for handling the unique demands of storage server-based ML tasks. 

Data in SALT is typically distributed across multiple drives. To facilitate efficient computation, SALT employs peer-to-peer technology for transferring data from regular disks to CSDs. Subsequent to this data movement, clustering is performed using the k-means++ algorithm~\cite{kmeanspp}. The integration of the `pread` system call with io\_uring~\cite{iouring} is a crucial aspect of our design, enabling parallel I/Os to efficiently transfer all requisite files to the compute server. Upon receipt of these files, the compute server embarks on the training process.

\subsection{Computational Efficiency and Sustainability}
An essential aspect of the SALT design is the focus on computational efficiency and sustainability. The choice of lattice-based encryption over RSA, despite the latter's maturity and performance benefits, is driven by the imperative of quantum-safe cryptography. The use of FPGA for both encryption/decryption and CNN acceleration underscores our commitment to energy-efficient computing. This approach is particularly vital in light of the significant energy and carbon footprint associated with DNN training~\cite{DNNcarbon01,DNNcarbon02,DNNcarbon03}. By optimizing both the hardware and software components for energy efficiency and minimizing unnecessary data movement, SALT sets a new benchmark in sustainable design for storage servers in ML applications.

\textbf{\textit{In summary, the SALT storage system presents an innovative approach to integrating storage and computation in machine learning environments. By marrying the efficiencies of FPGA-based lattice encryption with systolic array-based CNN accelerators and optimizing data movement through advanced system calls, SALT achieves a harmonious balance between computational efficiency, sustainability, and robust machine learning capabilities. This integration not only enhances the performance of storage servers, but also contributes significantly to the sustainability of large-scale machine learning operations.}}

%%%%%



